Quantum Leptogenesis I

Thermal leptogenesis explains the observed matter-antimatter asymmetry of the universe in terms of neutrino masses, consistent with neutrino oscillation experiments. We present a full quantum mechanical calculation of the generated lepton asymmetry based on Kadanoff-Baym equations. Origin of the asymmetry is the departure from equilibrium of the statistical propagator of the heavy Majorana neutrino, together with CP violating couplings. The lepton asymmetry is calculated directly in terms of Green's functions without referring to "number densities". Compared to Boltzmann and quantum Boltzmann equations, the crucial difference are memory effects, rapid oscillations much faster than the heavy neutrino equilibration time. These oscillations strongly suppress the generated lepton asymmetry, unless the standard model gauge interactions, which cause thermal damping, are properly taken into account. We find that these damping effects essentially compensate the enhancement due to quantum statistical factors, so that finally the conventional Boltzmann equations again provide rather accurate predictions for the lepton asymmetry.

==> erratum.tex <==
\thispagestyle{empty}
\noindent
{\bf\Large Erratum}\\
%

%\noindent
%In the following we list several errors contained in our paper.\\

1. Starting from Eq.~(2.11), $f_{Li}$ has to be replaced by $f_{Li}/2$;
starting from Eq.~(5.38), $L_{{\bf k}ii}$ has to be replaced by 
$L_{{\bf k}ii}/2$. In Eq.~(3.25) $P_L$ has to be replaced by $P_L\gamma^0$;
in Eq.~(5.33) $M$ has to be dropped; in the trace of Eq.~(5.34) a factor
$P_L$ has to be included; 
in Eqs.~(5.19), (5.20) and (5.45) the sign on the r.h.s.
has to be reversed. In Eqs.~(C.14) and (C.15) $dk'$ has to be replaced by 
$k'dk'$; in the first line of Eq.~(C.18) the 
$\varphi'$-integral has to be dropped and in the second line a factor $2\pi$
has to be included.

2. The statement after Eq.~(5.43), that $\mathcal{O}(t)$ does not contribute
to the asymmetry to leading order in $\Gamma$, is not correct. The leading 
contribution is given by
\begin{align}
L'_{{\bf k}ii}(t,t) =  -\epsilon_{ii}\ 16\pi 
&\int_{\bf q,q'} \frac{k\cdot k'}{kk'\omega_{\bf p}}\ f_N^{eq}(\omega_{\bf p}) 
f_{l\phi}(k,q) f_{l\phi}(k',q')
\frac{1}{(\Omega_1^2+\frac{\Gamma^2}{4})
(\Omega_3^2 +\frac{\Gamma^2}{4})} \nonumber \\ 
&\times\frac{2\Omega_1\Omega_3 +\frac{\Gamma^2}{2}}{\Omega_2}
\left(\sin(\Omega_2 t) - e^{-\frac{\Gamma t}{2}}\left(\sin(\Omega_1 t)
-\sin(\Omega_3 t)\right)\right) \ .
\end{align}
Changing integration variables, as
described in detail in Appendix~C (cf. Eq.~(C.19) and the following
discussion), one obtains
\begin{align}
L'_{{\bf k}ii}(t,t) =  &-\frac{\epsilon_{ii}}{2\pi^3\Gamma}\frac{1}{k} 
\int_{p_{\rm min}(k)}^{\infty}dp \int_{k'_{\rm min}(p)}^{k'_{\rm max}(p)}k'dk'
\int_{z_1^{\rm min}}^{z_1^{\rm max}}dz_1
\int_{z_3^{\rm min}}^{z_3^{\rm max}}dz_3
\frac{1}{\omega_{\bf p}}\nonumber\\
&\times\left(1-\frac{p^2+k^2-q^2}{2pk}\frac{p^2+k'^2-q'^2}{2pk'}\right) 
f_{l\phi}(k,q) f_{l\phi}(k',q') f_N^{eq}(\omega_{\bf p})\\
&\times\frac{1}{\left(z_1^2+1\right)\left(z_3^2+1\right)}
\frac{z_1 z_3 +1}{z_1 - z_3}
\left(\sin((z_1 - z_3)\tfrac{\tau}{2}) - 
e^{-\tfrac{\tau}{2}}\left(\sin(z_1\tfrac{\tau}{2})
-\sin(z_3\tfrac{\tau}{2})\right)\right) , \nonumber
\end{align}
where $\tau=\Gamma t$, $q=\omega_{\bf p} - k - \Gamma z_1/2$,
$q'=\omega_{\bf p} - k' - \Gamma z_3/2$ and
$z_{1,3}^{\rm min}=2\Omega_{1,3}^{\rm min}/\Gamma$,  
$z_{1,3}^{\rm max}=2\Omega_{1,3}^{\rm max}/\Gamma$,
with $z_{1,3}^{\rm min} < 0$ and $z_{1,3}^{\rm max} > 0$. In the limit 
$\Gamma/M \rightarrow0$ with $\tau=\Gamma t$ fixed, the integration limits 
approach $z_{1,3}^{\rm min} \rightarrow -\infty$ and 
$z_{1,3}^{\rm max} \rightarrow +\infty$, respectively. The integral can now 
be evaluated by means of Cauchy's theorem yielding the result 
\begin{align}
L'_{{\bf k}ii}(t,t) \rightarrow  
&-\frac{\epsilon_{ii}}{2\pi}\frac{1}{k} 
\int_{p_{\rm min}(k)}^{\infty}dp \int_{k'_{\rm min}(p)}^{k'_{\rm max}(p)}k'dk'
\frac{1}{\omega_{\bf p}} 
\left(1-\frac{2\omega_{\bf p} k-M^2}{2pk}
\frac{2\omega_{\bf p} k'-M^2}{2pk'}\right) \nonumber\\
&\times f_{l\phi}(k,\omega_{\bf p}-k)f_{l\phi}(k,\omega_{\bf p}-k')
f_N^{eq}(\omega_{\bf p})\frac{1-e^{-\tau}}{\Gamma}\ ,
\end{align}
which, up to the statistical factor, agrees with the Boltzmann result (C.15).
Hence, contrary to statements in the paper, the Boltzmann result is also
obtained for vanishing thermal damping widths in the limit 
$\Gamma \rightarrow 0$.\\


\noindent
We thank Mathias Garny for pointing out to us that  $\mathcal{O}(t)$ yields
the Boltzmann result in the zero-width limit.
